Skyline variations allow estimating distance to trees on landscape photos using semantic segmentation

Approximate distance estimation can be used to determine fundamental landscape properties including complexity and openness. We show that variations in the skyline of landscape photos can be used to estimate distances to trees on the horizon. A methodology based on the variations of the skyline has been developed and used to investigate potential relationships with the distance to skyline objects. The skyline signal, defined by the skyline height expressed in pixels, was extracted for several Land Use/Cover Area frame Survey (LUCAS) landscape photos. Photos were semantically segmented with DeepLabV3+ trained with the Common Objects in Context (COCO) dataset. This provided pixel-level classification of the objects forming the skyline. A Conditional Random Fields (CRF) algorithm was also applied to increase the details of the skyline signal. Three metrics, able to capture the skyline signal variations, were then considered for the analysis. These metrics shows a functional relationship with distance for the class of trees, whose contours have a fractal nature. In particular, regression analysis was performed against 475 ortho-photo based distance measurements, and, in the best case, a R2 score equal to 0.47 was achieved. This is an encouraging result which shows the potential of skyline variation metrics for inferring distance related information.

==> skyvar.tex <==
The output of the segmentation process is the discrete signal:
%
\begin{equation}
	y_{sky}[x] \qquad \mbox{for } 0 \leq x < W,
\label{eq:sky_sig}
\end{equation}
%
which takes values in the set, $\{0, H\}$, where $W$ and $H$ are the width and height of the original image. For each $x$ value, $y_{sky}[x]$ is the height of the skyline in the image. 
%
The second signal indicates to which class pixel $(x, y_{sky}[x])$ belongs. It and can be expressed as:
%
\begin{equation}
	c[x] = \sum_{k = 0}^{Nx-1}c_k\Pi_{D_k}[x - x_{c,k}]
	\label{eq:class_sig}
\end{equation}
%
where $c_k$ is the $k$th class value and $\Pi_{D_k}[x - x_{c,k}]$ is the casual unit door defined as
%
\begin{equation}
	\Pi_{D_k}[x - x_{c,k}] = \left\{
		\begin{array}{lr}
		1 & \mbox{for } x_{c,k} \leq x < x_{c,k} + D_k\\
		0 & \mbox{otherwise}.
		\end{array}
	\right.
	\label{eq:unit_door}
\end{equation}
%
$N_x$ is the number of objects defining the skyline. In this way, $c[x]$ is piece-wise constant on intervals of type, $[x_{c,k}, x_{c,k} + D_k)$. Each interval defines a skyline segment for which an object belonging to class $c_k$ has been identified.\\
%
These signals are shown in \fref{fig:signals}: $c[x]$ is depicted at the bottom of the figure as bar where each color represents a different class. 
\begin{figure}
	\centering
	\includegraphics[width=0.7\columnwidth]{images/signals}
	\caption{The skyline and classification signals extracted from a \acs{LUCAS} image.}
	\label{fig:signals}
\end{figure}
%
From this representation the piece-wise nature of the signal clearly appears.\\
In several images, it has been observed that the skyline is affected by variations not due to the shape of the skyline objects but to geometric effects. For example, a line of trees can be slanted because it is placed along a sloped hill that introduces horizontal variations in addition to changes due to the shapes of the trees. These geometric variations can be significant and hide the actual effects of the objects. For this reason, first order differences have been computed:
%
\begin{equation}
\dot{y}_{sky}[x] = y_{sky}[x] - y_{sky}[x-1] \quad \mbox{for } 1 \leq x < W.
\label{eq:first_order}
\end{equation}
%
By performing first order differences, which is approximately equivalent to compute a derivative, all linear trends present in $y_{sky}[x]$ are removed.
$\dot{y}_{sky}[x]$ and $c[x]$ are the basic signals used in the following for the computation of metrics quantifying the variability of the skyline.
%
\subsection{Variability metrics}
\label{ssec.metrics}
As discussed in \secref{ssec.refdata}, a data set of more than $450$ points with associated distances has been created. For each point, identified by the the coordinates $(x_i, y_i)$ with $y_i = y_{sky}[x_i]$, it is necessary to compute a metric, $m_i$, to quantify the variability of the corresponding skyline profile. In order to do so, the class of the point is at first identified using \eqref{eq:class_sig}. This class is denoted as $c_i = c[x_i]$. The boundaries of the corresponding skyline object are also determined as 
%
\begin{equation}
\begin{split}
    x_{c,i} &= \max\left\{x_{c,k} \leq x_i\right\}\\
    D_{i} &= x_{c,{i+1}} - x_{c,i}\\
    \label{eq:point_boundaries}
\end{split}
\end{equation}
%
where $x_{c,k}$ and $D_k$ have been defined above. $x_{c,i}$ and $D_i$ defines the range of points belonging to the same class of $x_i$: only these points will be used for the metric computation. Several metrics are considered in the following. These metrics have been selected since they are typical indicators used in the literature to quantify the variability of a signal.
%
\subsubsection{\ac{NSL}}
This is the original metric proposed by \cite{Aifantopoulou2007} and adapted here to individual objects forming the skyline. This metric is computed for the $i$th object as:
%
\begin{equation}
\begin{split}
m_{nsl,i} &= \frac{1}{D_i - 1}\sum_{x_{c,i} + 1}^{x_{c,i} + D_i - 1}\sqrt{(y_{sky}[x] - y_{sky}[x-1])^2 + 1^2} \\
		  &= \frac{1}{D_i - 1}\sum_{x_{c,i} + 1}^{x_{c,i} + D_i - 1}\sqrt{\dot{y}_{sky}[x]^2 + 1}.
\end{split}
\label{eq:norm_length}
\end{equation}
%
The total length is computed as sum of the lengths of the individual segments obtained by considering subsequent pixels. The two terms under square root are the 
horizontal and vertical variations between consecutive pixels. For this reason, the horizontal variation is always equal to $1$. $m_{nsl,i}$ depends only on $\dot{y}_{sky}[x]$ and is normalized by $D_i - 1$, the length that would be obtained if $y_{sky}[x] = 0$ for all $x$.
%   
\subsubsection{Sample variance}
%
The second metric considered for the analysis is the sample variance of $\dot{y}_{sky}[x]$ defined as \cite{Casella2001}:
%
\begin{equation}
    m_{sv,i} = \frac{1}{D_i - 1}\sum_{x = x_{c,i} + 1}^{x_{c,i} + D_i - 1}\left(\dot{y}_{sky}[x] - \overline{\dot{y}_{sky}}\right)^2
    \label{eq:variance}
\end{equation}
%
where $\overline{\dot{y}_{sky}}$ is the sample mean:
%
\begin{equation}
    \overline{\dot{y}_{sky}} = \frac{1}{D_i-1}\sum_{x = x_{c,i} + 1}^{x_{c,i} + D_i - 1}\dot{y}_{sky}[x].
    \label{eq:sample_mean}
\end{equation}
%
Note that both sample variance and mean are computed considering samples in the interval $[x_{c,i}, x_{c,i} + D_{i} - 1]$, i.e. using samples belonging to the same object class. Moreover,
%
\begin{equation}
	\begin{split}
\overline{\dot{y}_{sky}} &= \frac{1}{D_i-1}\sum_{x = x_{c,i} + 1}^{x_{c,i} + D_i - 1}\left(y_{sky}[x] - y_{sky}[x-1]\right)\\
&= \frac{1}{D_i-1}\left[\sum_{x = x_{c,i} + 1}^{x_{c,i} + D_i - 1}y_{sky}[x] - \sum_{x = x_{c,i}}^{x_{c,i} + D_i - 2}y_{sky}[x]\right]\\
&= \frac{1}{D_i-1}\left(y_{sky}[x_{c,i}+D_i-1] - y_{sky}[x_{c,i}]\right) 
	\end{split}
\label{eq:sample_mean_2}
\end{equation}
%
For large values of $D_i$ and small signal variations, $\overline{\dot{y}_{sky}} \approx 0$ and
%
\begin{equation}
	m_{sv,i} \approx \frac{1}{D_i - 1}\sum_{x = x_{c,i} + 1}^{x_{c,i} + D_i - 1}\left(y_{sky}[x] - y_{sky}[x-1]\right)^2
	\label{eq:variance_2}
\end{equation}
%
which is a form of \ac{AVAR} \cite{Allan1966}.
%
\subsection{Average absolute deviation}
\eqref{eq:variance_2} suggests others variability metrics where different powers of signal differences are considered. In particular, \eqref{eq:variance_2} can be generalized as
%
\begin{equation}
m_{p,i} = \frac{1}{D_i - 1}\sum_{x = x_{c,i} + 1}^{x_{c,i} + D_i - 1}\left|y_{sky}[x] - y_{sky}[x-1]\right|^p = \frac{1}{D_i - 1}\sum_{x = x_{c,i} + 1}^{x_{c,i} + D_i - 1}\left|\dot{y}_{sky}[x]\right|^p
\label{eq:power_p}
\end{equation}
%
While we have analysed different values of $p$, in the following only the case $p = 1$ is analysed. This value led to the most promising results along with the sample variance. For $p =1$, $m_{1,i}$ represents the average absolute deviation of $\dot{y}_{sky}[x]$. 
%
\subsubsection{Windowed metrics}
\label{sssec.wm}
%
The metrics described above can be interpreted as averages computed considering a whole segment over which a single object class was detected. Windowed version of such metrics can be computed by limiting the duration of the summations in the metric computation.  The windowing process adopted to generalize the skyline metrics is illustrated in \fref{fig:windowing}.
%
\begin{figure}
	\centering
	\includegraphics[width=0.8\columnwidth]{images/windowing}
	\caption{Schematic representation of the windowing process adopted to generalize dispersion sky-line metrics.}
	\label{fig:windowing}
\end{figure}
%
In this case, the different metrics are computed as:
%
\begin{equation}
m_{i}(L) = \frac{1}{x_{U,i} - x_{L,i} - 1}\sum_{x = x_{L,i} + 1}^{x_{U,i} - 1}f\left(\dot{y}_{sky}[x]\right)
\label{eq:windowed_metrics}
\end{equation}
%
where
\begin{itemize}
	\item $L$ is the length of the analysis window
	\item 
	\[
		x_{L,i} = \max\left(x_{c,i}, x_i - \lfloor L/2\rfloor \right)
	\]
	\item
	\[
		x_{U,i} = \min\left(x_{c,i} + D_i, x_i + \lfloor L / 2\rfloor \right)
	\]
	\item $f(\cdot)$ is used to denote the generic function used for the metric computation. For example, for the metric in \eqref{eq:power_p}, $f(\cdot) = |\cdot|^p$.
\end{itemize}
As previously defined, $x_i$ is the horizontal coordinate of the reference point for which the metric is computed.\\
%
As it will be shown in the result section, windowing can improve the ability of the metrics in mapping the distance to skyline objects. The rationale of applying windowing is to limit the effects of objects at different distances in the metrics computation. Consider for example, a skyline made of a line of trees. These trees could be aligned in a slanted way and have different distances from the camera. Without windowing, all the skyline points of this line of trees will be used for the metric computation since they all belong to the same class (trees). However, a hypothetical reference point $x_i$ refers to a single tree with a specific distance from the camera. Windowing reduces the impact of contamination of the nearby trees in the metric computation selecting a maximum of $L$ points around $x_i$.\\
%
Windowing also reduces the occurrence of duplicated metric values. Consider the case where two reference points in the same image belong to the same object. This could happen for example when both a chimney and the top of a roof are selected when considering the same house profile. Since the two points belong to the same object, they will lead to the very same metric value if windowing is not applied. In such a case, two different distance values will be associated to the same metric. Windowing is thus introduced also to reduce this effect. 
~\\
In the following, the three metrics described above and their windowed versions will be considered for a total of $6$ metrics. While other metrics were considered, they are not discussed since they did not show a dependency with respect to the camera distance.     
%
\subsection{Metric-to-Distance Models}
\label{ssec.models}
%
The metrics discussed above have been computed using the reference data generated according to the procedure discussed in \secref{ssec.refdata} and plotted as a function of the measured distances, $d_i$. In this way, scatter plots have been obtained. When both $m_i$ and $d_i$ are plotted in logarithmic scale, a linear trend was observed. In the following, symbol $m_i$ is used to denote a generic metric: the appropriate subscript is used to indicate specific quantities.\\
%
While the scatter plots obtained for the different metrics will be better discussed in \secref{sec.results}, the linear trends observed when logarithmic scales are adopted suggested the use of linear models for regression analysis \cite{Casella2001,Draper1998}:
%
\begin{equation}
\log(m_i) = \alpha + \beta\log(d_i).
\label{eq:log_linmodel}
\end{equation}
%
This model implies a power law between $m_i$ and $d_i$,
%
\begin{equation}
m_i = \mbox{e}^\alpha d_i^\beta = k\cdot d_i^\beta.
\label{eq:powerlaw_model}
\end{equation}
%
In the following, regression analysis using model \eref{eq:log_linmodel} is performed. The goodness of the regression is assessed using the coefficient of determination, $R^2$ \cite{Casella2001,Draper1998}.\\
Where appropriate, the following simplified model will also be considered in addition to \eqref{eq:powerlaw_model}:
%
\begin{equation}
m_i = \frac{k}{d_i}.
\label{eq:inverse_power}
\end{equation}
%
This model implies that the level of variations (length) of fractal curve increases with the inverse of distance.   
